Eccentric Binary Black Hole Simulations with Numerical Relativity

We perform a systematic study of eccentric orbiting nonspinning black hole binaries. We first make a technical study of the optimal full numerical techniques to apply to these studies. We choose different gauge parameters and Courant factors, $c=dx/dt$, and find an optimal value for it of 0.45. We also find the grid structure and global resolution that optimize accuracy and speed of current computational resources. With these choices we perform a study of the merger times $t_m$ as a function of eccentricity for configurations with comparable orbital energy content and find that they are well represented by the post-Newtonian factor $F(e)=(1+73e^2/24+37e^4/96)/(1-e^2)^{7/2}$ when merger times are normalized to their quasicircular values, i.e. $t_m(e)/t_m\approx F(e)$. We then perform a systematic coverage of five small-medium eccentricities up to $e\sim0.45$ and six mass ratios up to 8.5:1 producing a total of 30 simulations covering up to 25 orbits to merger to further model merger times and as a seed to a forthcoming new systematic catalog of gravitational waveforms from eccentric binary black holes to directly perform parameter estimations of gravitational waves events.

==> grid_q1_convergence_table.tex <==
\begin{table}
\caption{Number of refinement levels and respective size used in the equal-mass convergence simulations. For each resolution and level, we also report the spatial step d$x$, all in units of $M=m_1^H+m_2^H$.\label{tab:eBBH_q1_grid_convergence}}
\begin{tabular}{ccccc}
\hline
level & size & $n$100 d$x$ & $n$120 d$x$ & $n$144 d$x$ \\
\hline
0 & 400 & 4.00 & 3.33 & 2.78 \\
1 & 208 & 2.00 & 1.67 & 1.39 \\
2 & 115 & 1.00 & 0.83 & 0.69 \\
3 & 36  & 0.50 & 0.416 & 0.347 \\
4 & 12  & 0.25 & 0.208 & 0.174 \\
5 & 4   & 0.125 & 0.104 & 0.087 \\
6 & 2   & 0.0625 & 0.0521 & 0.0434 \\
7 & 1   & 0.0313 & 0.0260 & 0.0217 \\
\hline
\end{tabular}
\end{table}


==> overlap_extraction_radii.tex <==
%\begin{table}
%\label{tab:matching_extrapolation}
%\caption{Matching overlaps between extrapolated waveforms at infinity computed from different extraction radii.}
%\begin{tabular}{l|ccc}
%\toprule
%($R_{1},R_{2}$) & (75,113) & (75,185) & (113,185)\\
%\hline
%full & 0.997207922 & 0.995934771 & 0.999834079 \\
%inspiral & 0.904718546 & 0.897740258 & 0.997922186 \\
%merger & 0.999992614 & 0.999229369 & 0.999269955 \\
%\hline
%\end{tabular}
%\end{table}

\begin{table}
\label{tab:matching_extrapolation}
\caption{Matching overlaps between extrapolated waveforms at infinity computed from different extraction radii.}
\begin{tabular}{l|ccccccc}
\toprule
($R_{1},R_{2}$) & (75,113) & (75,185) & (75,270) & (113,185) & (113,270) & (185,270) & (113,496) \\
\hline
full & 0.9972 & 0.9959 & 0.9956 & 0.9998 & 0.9997 & 0.9999 & 0.9969 \\
inspiral & 0.9491 & 0.9380 & 0.9416 & 0.9982 & 0.9994 & 0.9993 & 0.9884 \\
merger & 0.9999 & 0.9992 & 0.9968 & 0.9993 & 0.9968 & 0.9990 & 0.9994 \\
\hline
\end{tabular}
\end{table}

